Solarcast-ML: Per Node GraphCast Extension for Solar Energy Production

This project presents an extension to the GraphCast model, a state-of-the-art graph neural network (GNN) for global weather forecasting, by integrating solar energy production forecasting capabilities. The proposed approach leverages the weather forecasts generated by GraphCast and trains a neural network model to predict the ratio of actual solar output to potential solar output based on various weather conditions. The model architecture consists of an input layer corresponding to weather features (temperature, humidity, dew point, wind speed, rain, barometric pressure, and altitude), two hidden layers with ReLU activations, and an output layer predicting solar radiation. The model is trained using a mean absolute error loss function and Adam optimizer. The results demonstrate the model's effectiveness in accurately predicting solar radiation, with its convergence behavior, decreasing training loss, and accurate prediction of solar radiation patterns suggesting successful learning of the underlying relationships between weather conditions and solar radiation. The integration of solar energy production forecasting with GraphCast offers valuable insights for the renewable energy sector, enabling better planning and decision-making based on expected solar energy production. Future work could explore further model refinements, incorporation of additional weather variables, and extension to other renewable energy sources.

==> holding.tex <==
Data was collected from the Copernicus system.

Requests are fielded against the offline database, take approximately 30 minutes per data request.

https://cds.climate.copernicus.eu/cdsapp#!/yourrequests?tab=form

Dataset required approximately 30kb per day.  Can only download 4 days at a time.

Dataset was zeroed on the area for which the ground truth was availble.  The grid layout matched the original GraphCast (?)

Lat and log for the datapoint was 42.56000137, -83.63999939

The distance from the ground truth location to the training location was 481ft.

Data was validated from the NC files supplied from Copernicus back against commercially available almanacs.

Data was validated using the Panoply tool made available from NASA.


